From Market Saturation to Social Reinforcement: Understanding the Impact of Non-Linearity in Information Diffusion Models

Diffusion of information in networks is at the core of many problems in AI. Common examples include the spread of ideas and rumors as well as marketing campaigns. Typically, information diffuses at a non-linear rate, for example, if markets become saturated or if users of social networks reinforce each other's opinions. Despite these characteristics, this area has seen little research, compared to the vast amount of results for linear models, which exhibit less complex dynamics. Especially, when considering the possibility of re-infection, no fully rigorous guarantees exist so far. We address this shortcoming by studying a very general non-linear diffusion model that captures saturation as well as reinforcement. More precisely, we consider a variant of the SIS model in which vertices get infected at a rate that scales polynomially in the number of their infected neighbors, weighted by an infection coefficient $\lambda$. We give the first fully rigorous results for thresholds of $\lambda$ at which the expected survival time becomes super-polynomial. For cliques we show that when the infection rate scales sub-linearly, the threshold only shifts by a poly-logarithmic factor, compared to the standard SIS model. In contrast, super-linear scaling changes the process considerably and shifts the threshold by a polynomial term. For stars, sub-linear and super-linear scaling behave similar and both shift the threshold by a polynomial factor. Our bounds are almost tight, as they are only apart by at most a poly-logarithmic factor from the lower thresholds, at which the expected survival time is logarithmic.

==> content/conclusion.tex <==
We conducted the first fully rigorous analysis of the SIS model with non-linear infection rates in the number of infected neighbors.
Our results provide almost-tight lower and upper bounds on the epidemic threshold for both star and clique graphs. Those are important graph classes because they provide insights for the two extremes of very little connectivity and full connectivity, respectively. Moreover, since we consider the SIS process, survival time lower bounds also carry over to graphs that contain those classes as sub graphs. Hence, our lower bounds carry over to graphs with very high degree vertices.

On cliques with sub-linear scaling, the process behaves very similar to the normal SIS process and the threshold only shifts by a poly-logarithmic factor. When the infection scales super-linearly, the process completely changes as at the threshold, there exists an equilibrium point that is repellent. That means that the process dies out very fast asymptotically almost surely but if it reaches the equilibrium, it survives so long that the overall expected survival time is still exponential. The threshold in this setting is by a polynomial factor smaller than in the sub-linear case. On stars, we show that sub-linear and super-linear scaling do not differ that much and the threshold changes by a polynomial factor that depends on the scaling of the infection.

As a next step it is very interesting to see to which extend these results carry over to larger graph classes or even real-world graphs. A starting point for that could be running experiments on such graphs. For further theoretical results, we believe that expansion is the most promising property to analyze. That would give results for a lot of graph classes like Erdős--Rényi graph. High expansion results in a very good bound on the number of edges between susceptible and infected vertices. In the standard SIS model, this translates to a bound on the rate at which vertices get infected. However, in our model, this is not immediate, as the rate at which vertices get infected also depends on how their edges are distributed. It makes a difference whether all susceptible vertices have roughly the same number of infected neighbors or whether some of them have many more than others. This makes our model harder to analyze than the standard model.

Another direction would be to look at more advanced infection models like the SIRS model, which adds temporary immunity to the process, and adjust those in the same way to non-linear infection rates. That gives a better understanding into under which conditions the adjusted scaling makes a difference and how much of a difference it is.

The adjusted infection function can model infections that scale polynomially with the number of infected neighbors. It would be interesting to also look into other functions like for example threshold functions that stay at 0 until a specific threshold is reached and only then start increasing.
